Zip-zip Trees: Making Zip Trees More Balanced, Biased, Compact, or Persistent

We define simple variants of zip trees, called zip-zip trees, which provide several advantages over zip trees, including overcoming a bias that favors smaller keys over larger ones. We analyze zip-zip trees theoretically and empirically, showing, e.g., that the expected depth of a node in an $n$-node zip-zip tree is at most $1.3863\log n-1+o(1)$, which matches the expected depth of treaps and binary search trees built by uniformly random insertions. Unlike these other data structures, however, zip-zip trees achieve their bounds using only $O(\log\log n)$ bits of metadata per node, w.h.p., as compared to the $\Theta(\log n)$ bits per node required by treaps. In fact, we even describe a ``just-in-time'' zip-zip tree variant, which needs just an expected $O(1)$ number of bits of metadata per node. Moreover, we can define zip-zip trees to be strongly history independent, whereas treaps are generally only weakly history independent. We also introduce \emph{biased zip-zip trees}, which have an explicit bias based on key weights, so the expected depth of a key, $k$, with weight, $w_k$, is $O(\log (W/w_k))$, where $W$ is the weight of all keys in the weighted zip-zip tree. Finally, we show that one can easily make zip-zip trees partially persistent with only $O(n)$ space overhead w.h.p.

==> external.tex <==
\section{Introduction}
The \emph{zip tree} is a randomized binary search tree introduced by Tarjan,
Levy, and Timmel~\cite{zip} that organizes a set of $n$ distinct keys in a
simple way, where
keys are organized left-to-right according to 
increasing keys (in inorder) and internally according to a max-heap order
for small 
random \emph{ranks} that are assigned to the keys.

At a high level, zip trees are 
similar to 
the random \emph{treap} data structure
of Seidel and Aragon~\cite{treaps} and the \emph{skip list} data structure
of Pugh~\cite{skip-lists}, but with several advantages.
For example,
insertions and deletions in zip trees are described in terms of simple ``zip''
and ``unzip'' operations rather than sequences of 
rotations, as in treaps, which are arguably more complicated.
Like treaps, zip trees organize keys using random ranks, but the ranks used
by zip trees are $\Theta(\log \log n)$-bit ranks, whereas the ranks
used by treaps are $\Theta(\log n)$-bit ranks.
Also,
as we review and expand upon, zip trees are topologically isomorphic to
skip lists, but use significantly less space than skip lists.

Like treaps and skip lists, zip trees 
have an advantage related to privacy preservation, which is known
as \emph{history independence}, e.g., see~\cite{hartline}.
For example, a data structure is said to be \emph{weakly history independent}
if, for any two sequences of operations $X$ and $Y$ that take
the data structure from initialization to state $A$, 
the distribution over memory after $X$ is
performed is identical to the distribution after $Y$.
Thus, if an adversary observes the final state of the data structure,
the adversary cannot determine the sequence of operations that lead to 
that state.
A data structure 
is \emph{strongly history independent}, on the other hand,
if, for any two (possibly empty) sequences of operations
$X$ and $Y$ that take a data structure in state $A$ to state $B$, the distribution over representations
of $B$ after $X$ is performed on a representation, $r$, is identical to the distribution after $Y$ is
performed on $r$.
Thus, if an adversary observes the states of the data structure
at different times,
the adversary cannot determine the sequence of operations that lead to 
the second state beyond just what can be inferred from the states themselves.

In this paper, we show how the inherent advantages of zip trees over 
other randomized data structures lead to simple new extensions and
generalizations of zip trees, which we refer to as \emph{zip tree cultivars}.
Zip tree cultivars that we study include the following:
\begin{itemize}
\item
\emph{canonical zip trees}: These are the original variety of zip trees,
which have expected height $1.5\log n$ and are strongly history independent.
\item
\emph{multiway zip trees}: These are a multiway variety of zip trees, 
where we don't restrict the number of children for each internal node,
which have expected height $\log n + 3$ and are strongly 
history independent.
Canonical zip trees can be derived from multiway zip trees by replacing 
each subtree of nodes of the same rank with a right-heavy path.
\item
\emph{uniform zip trees}: These are binary zip trees that can be derived
from multiway zip trees by replacing each subtree of nodes of the same
rank with a binary subtree of the same size where all such trees are equally
likely.
Uniform zip trees have expected height $1.339\log n$ 
[\todo{xxx Double-check} xxx] and are weakly history independent.
\item
\emph{fusion zip trees}: These are
internal-memory word-RAM zip-tree structures that take advantage of the
$O(\log\log n)$-bit ranks of zip trees to support
insertions, deletions, and searches in $O(\log n/\log\log n)$ time
with high probability.
\item
\emph{zip B-trees}: these are simple external-memory versions of 
zip trees that
support searches and updates in $O(\log_B n)$ time, 
with high probability, where
$B$ is the block size used for input/output (I/O) operations from/to 
external memory.
We further subdivide these types of zip trees 
depending on whether they perform partitioning into blocks
according to a ``partition-by-size'' (PBS) or 
a ``partition-by-rank'' (PBR) rule.
For instance, if we use partition-by-size, we get a strongly 
history-independent version of zip B-trees.
One consequence of this, however, is that
PBS external zip trees use linear space, w.h.p., for most but not all 
possible values for the parameter, $B$.
In contrast, PBR external zip trees always use linear space, but only
guarantee weak history indepence rather than
strong history independence.
\item
\emph{weighted zip trees}:
These are
weighted versions of zip trees, 
which support searches with performance bounds that 
are logarithmic in $W/w_k$, where $W$ is the total weight of all keys 
in the tree and $w_k$ is the weight of the search key, $k$.
As we show, this, in turn,
allows weighted 
zip trees to be used in simplified versions of the link-cut tree
data structure of Sleator and Tarjan~\cite{link-cut} for dynamically
maintaining arbitrary trees.
\end{itemize}

As with canonical zip trees, all the above zip-tree cultivars utilize
$O(\log\log n)$ bits of metadata for each key, particularly if they
are implemented using the tiny pointers 
technique
of Bender, Conway, Farach-Colton, Kuszmaul, 
and Tagliavini~\cite{tiny-pointers}.

In addition, we show how isomorphisms between 
zip trees and skip lists can be
used to analyze our different zip-tree cultivars.



==> skip-trees.tex <==
\subsection{Skip Trees}
A \emph{skip tree}, $T$, is a multiway tree that is dual to a corresponding skip
list, $L$; see, e.g., Dean and Jones~\cite{duality}.
The root, $r$, of $T$ corresponds to the interval, $(-\infty,+\infty)$, of 
the highest level of $L$, and it stores the keys, $-\infty$ and $+\infty$.
We create a node, $v$ in $T$, for every other maximal 
non-empty sublist $L_{i,j}$ on
level $i$ in $L$ between two keys, $k_1$ and $k_2$, 
that also appear in level $i+1$, and we
store all the keys in $L_{i,j}$ in $v$ and we define the interval
for $v$ to be $(k_1,k_2)$.
We then define the parent of $v$ to be the (unique) node, $w$ in $T$, 
that contains $k_1$ and $k_2$, and we link $w$ to $v$ as being the 
next place to search for any keys that fall in the interval $(k_1,k_2)$.
Define the \emph{rank} of a node, $v$, in a skip tree, $T$, as 
the (highest) level that all the keys stored in $v$ would 
have in the skip list dual to $T$, i.e., the key's height in the dual skip
list, which is equal to a draw from a geometric distribution with success
probability $1/2$.
(See \Cref{fig:skip-tree}.)

\begin{figure}[hbt]
\centering
\includegraphics[scale=.7, trim=2in 3.75in 2in 4in, clip]{figs/skip-tree.pdf}
\caption{\label{fig:skip-tree} An example skip tree, corresponding
to the skip list in \Cref{fig:skip}. 
\todo{This is stolen from Dean and Jones. Make a new figure, which has
$-\infty$ and $+\infty$, not $r$, and no edge weights. Show ranks,
not rank differences.}}
\end{figure}

The following lemma follows immediately from well-known facts about
skip lists, but it is nevertheless useful for our purposes.
Let $n(v)$ denote the number of keys stored in a node, $v$, in a skip tree.

\begin{lemma}
\label{lem:skip-group}
If $v$ is a node in a skip tree, $T$, then $E[n(v)]=2$. 
Further, for any $n>1$ and constant $c\ge 1$, 
$\Pr(n(v)\ge c\log n)\le n^{-c}$.
Also, the probability that the rank of the root of $T$ is more than
$\log n + f(n)$ is at most $2^{-f(n)}$.
\end{lemma}
\begin{proof}
By definition, each key stored in a node $v$ in a skip tree corresponds to
a key that is stored in a level $i$ in a skip list, but not in level $i+1$.
Moreover, in order for $v$ to exist as a node in $T$, $n(v)\ge 1$.
Thus, $n(v)=X$, where $X$
is a geometric random variable with success probability $1/2$,
which implies that $E[n(v)] = 2$.
Also, for the same reason,
$\Pr(n(v)\ge c\log n)\le 2^{-c\log n} = n^{-c}$.
The final claim follows directly from \Cref{thm:skip-max}.
\qed\end{proof}

We also have the following related fact.

\begin{theorem}
\label{thm:skip-depth}
The expected depth for any key, $k$, in a skip tree, $T$, storing
$n$ keys is at most $0.5\log n + O(1)$.
\end{theorem}
\begin{proof}
The proof follows from \Cref{lem:skip-group} and
Lemma~3.4 from Tarjan, Levy, and Timmel~\cite{zip}.
For completeness, we also include a proof in an appendix.
\qed\end{proof}


